DPLM-2: A Multimodal Diffusion Protein Language Model

Proteins are essential macromolecules defined by their amino acid sequences, which determine their three-dimensional structures and, consequently, their functions in all living organisms. Therefore, generative protein modeling necessitates a multimodal approach to simultaneously model, understand, and generate both sequences and structures. However, existing methods typically use separate models for each modality, limiting their ability to capture the intricate relationships between sequence and structure. This results in suboptimal performance in tasks that requires joint understanding and generation of both modalities. In this paper, we introduce DPLM-2, a multimodal protein foundation model that extends discrete diffusion protein language model (DPLM) to accommodate both sequences and structures. To enable structural learning with the language model, 3D coordinates are converted to discrete tokens using a lookup-free quantization-based tokenizer. By training on both experimental and high-quality synthetic structures, DPLM-2 learns the joint distribution of sequence and structure, as well as their marginals and conditionals. We also implement an efficient warm-up strategy to exploit the connection between large-scale evolutionary data and structural inductive biases from pre-trained sequence-based protein language models. Empirical evaluation shows that DPLM-2 can simultaneously generate highly compatible amino acid sequences and their corresponding 3D structures eliminating the need for a two-stage generation approach. Moreover, DPLM-2 demonstrates competitive performance in various conditional generation tasks, including folding, inverse folding, and scaffolding with multimodal motif inputs, as well as providing structure-aware representations for predictive tasks.

==> 020_related.tex <==
\section{Related Work}
\label{sec:related}


\subsection{Language Models}
% Language models learn with self-supervised objectives.
% This enables 
The dominant paradigm of language models is autoregressive language models, which breaks down the mutual distribution over the tokens of a sequence into conditional probabilities via the chain rule ${p(\bm{x}^{[1:N]})=\prod_{i=1}^N p(x^{[i]}|\bm{x}^{[1:i-1]})}$ and generates tokens by ancestral sampling from left to right~\citep{bengio2000neural,sutskever2014sequence,vaswani2017attention}.
Recently, researchers propose the non-autoregressive language models as an alternative~\citep{gu2018non}. 
These models do not need to obey the left to right generation order~\citep{qian2022diff,huang2022PDAT} and demonstrate competitive or superior performance compared to their autoregressive counterpart across a wide range of domains including languages~\citep{qian2021volctrans,huang2022PDAT,qian2022diff,huang2022PDAT,zheng2023reparameterized}, speeches~\citep{kim2021conditional}, proteins~\citep{zheng2023structure}, and molecules~\citep{hoogeboom2022equivariant}.
Among the numerous non-autoregressive language models, diffusion language models~\citep{li2022diffusionlm,gong2022diffuseq,zheng2023reparameterized} have emerged as a solid and promising framework.
Pretraining language models on a massive scale of unlabeled data markedly improves their downstream task performance~\citep{word2vec,elmo,radford2018gpt,devlin2019bert}.
As data volume and model sizes scale up, the training loss of language models predictably declines~\citep{kaplan2020scaling,hoffmann2022training,muennighoff2023scaling}, and enhancing downstream task performance even without specific tuning~\citep{gpt2}.
GPT3~\citep{brown2020gpt3} is a significant point in the journey, taking model sizes to 175B parameters, proposing in-context learning to bolster language models' competence in solving certain tasks with only a handful of demonstrations.
Furthermore, \citet{wei2021flanv1,t0,ouyang2022instructgpt} introduce instruction tuning, finetuning pretrained language models on series of tasks described via instructions, which elicits the instruction following ability of models and significantly enhances their zero-shot performance on unseen tasks.
More impressively, sufficiently large language models exhibit the emergent abilities such as multi-step reasoning~\citep{kojima2022zeroshotcot,wei2022emergent,wei2022CoT}, which small models do not possess~\citep{fu2023specializing}.
Empowered by large language models, helpful applications such as conversational AI systems\footnote{\url{https://chat.openai.com/}} and autonomous agents\footnote{\url{https://github.com/Significant-Gravitas/Auto-GPT}} have garnered much interest.
Although the most capable models at the moment are restricted in access, open-sourced efforts~\citep{zeng2022glm,touvron2023llama,touvron2023llama2,alpaca,vicuna2023,moss} have largely enhanced the public accessibility of powerful large language models.

\subsection{Protein Language Models}
% A large body of work has focused on modeling the sequences for proteins.
Thanks for the abundance of 1D amino acid sequences, there is growing interest in developing protein LMs at the scale of evolution, such as the series of ESM~\citep{rives2019esm,lin2022esmfold}, TAPE~\citep{rao2019evaluating}, 
ProtTrans~\citep{elnaggar2021prottrans}, PRoBERTa~\citep{nambiar2020transforming}, PMLM~\citep{he2021pre}, 
ProteinLM~\citep{xiao2021modeling}, 
PLUS~\citep{min2021pre}, 
Adversarial Masked LMs~\citep{mcdermott2021adversarial}, 
ProteinBERT~\citep{brandes2022proteinbert}, 
CARP~\citep{yang2022convolutions} in masked language modeling (MLM) paradigm, 
%ProtTrans~\citep{elnaggar2021prottrans}, 
ProtGPT2~\citep{ferruz2022protgpt2} in causal language modeling paradigm, and several others~\citep{melnyk2022reprogramming,madani2021deep,unsal2022learning, nourani2021tripletprot, lu2020self, sturmfels2020profile, strodthoff2020udsmprot}.
These protein language models exhibit remarkable generalization ability on various downstream tasks and be able to capture evolutionary information about secondary and tertiary structures from sequences alone.
Meanwhile, recent study shows these models' potency in revealing protein structures~\citep{lin2022esmfold}, predicting the effect of sequence variation on function~\citep{meier2021language}, antibody infilling~\citep{melnyk2022reprogramming} and many other general purposes~\citep{rives2019esm}.
Simultaneously, \citet{verkuil2022language} demonstrate that the large scale protein LMs can generate \textit{de novo} proteins by generalizing beyond natural proteins, both theoretically and experimentally validating their hypothesis in exhaustive detail, in which \pLMs demonstrate competency in designing protein structure despite being exclusively trained on sequences.

% Recently language models have been proposed for modeling large-scale databases of protein sequences rather than families of related sequences. Examples include (Bepler & Berger, 2019; Alley et al., 2019; Heinzinger et al., 2019; Rao et al., 2019; Madani et al., 2020; Elnaggar et al., 2021; Rives et al., 2021; Rao et al., 2021). Meier et al. (2021) found that the log-likelihoods of large protein language models predict mutational effects. Madani et al. (2021) study an autoregressive sequence model conditioned on functional annotations and show it can generate functional proteins.






%\paragraph{Language Modeling} aims to learn a probabilistic model to describe sequence data $p(\bm{x}^{[1:N]})$ of interest~\citep{shannon1951prediction,Jurafsky2009}. 


\subsection{Diffusion Language Models}
Derived from diffusion models~\citep{sohl2015diffusion}, diffusion language models is a variety of generative model that samples data via an iterative denoising process from noise. They can be divided into continuous~\citep{ho2020ddpm,song2020sde} and discrete~\citep{hoogeboom2021argmax,austin2021structured} categories according to the distribution they model.
Continuous diffusion models make great success in vision~\citep{dhariwal2021diffusionbeatgans,rombach2021highresolution,ho2022imagenvideo}, but they struggle in languages for operating on continuous surrogates of discrete tokens~\citep{li2022diffusionlm,gong2022diffuseq,han2022ssd,cdcd,yuan2022seqdiffuseq,gao2022difformer,ye2023dinoiser,chen2023cheaper,wu2023ar}, which has difficulty bypassing the pitfall of discreteness~\citep{ye2023dinoiser} and still lags behind autoregressive language models.
In contrast, discrete diffusion models, albeit having limited progress in large-scale applications, are innately suited to the data type inherent to languages (\ie, sequences of discrete tokens).
\citet{zheng2023reparameterized} makes commendable strides in discrete diffusion models and enhancing these models to yield comparable performance with autoregressive models on typical language generation benchmarks like machine translation.
Furthermore, as shown by \citet{he2022diffusionbert,zheng2023structure}, there are close relationship between discrete diffusion models and masked language models~(MLM), a widely adopted pretraining paradigm in NLP~\citep{devlin2019bert,liu2019roberta}.
% are closely related to trustworthy masked language models~\citep{ghazvininejad2019mask,he2022diffusionbert} and have 
% Inspired by these discoveries, in this work, we investigate the scalability of diffusion language models to explore their potential further.
Following this line, \citet{ye2023diffusion} propose scaling discrete diffusion LMs with diffusive adaptation, showing strong performance on several conditional text generation tasks, and accessing zero-shot instruction following, few-shot in-context learning and the promise of structured reasoning with instruction tuning.
% The most relevant work to ours is \citet{han2023ssd2} which builds a 13B chat model with continuous simplex-based diffusion language models.
% In contrast, our work focuses on discrete diffusion language models and their general abilities on diverse tasks.


\subsection{Protein Structure Diffusion Models}
Diffusion models have become popular tools in structural biology for protein generation, and their utility has been demonstrated across a range of generative tasks in recent years. \citet{trippe2022diffusion}, along with others, have introduced several diffusion model variants, each with its unique approach. For instance, while some models focus on generating the protein backbone by diffusing over protein coordinates, others, such as those proposed by \citet{wu2022high}, target inter-residue angles. \citet{lin2023generating} and \citet{yim2023framediff} have developed models that handle both the position and orientation of residue frames.
% An integrated approach to both sequence and structure generation has been explored by Lisanza et al. (2023), who presented a method that simultaneously produces sequence and backbone. Anand \& Achim (2022) have expanded on this to include side-chain atoms as well. Additionally, Latent Diffusion Models (LDMs) are gaining traction for various applications, including protein sequence synthesis by Jiang et al. (2023), protein backbone construction by Fu et al. (2023), and 3D molecule generation as demonstrated by Xu et al. (2023).
% All these methods utilize latent diffusion processes, adopting different techniques to construct a continuous latent space that effectively encodes input information. For example, one approach divides the latent space into invariant and equivariant components to represent molecules efficiently. The success of these methods in their respective tasks highlights the growing potential and benefits of applying latent diffusion techniques in the field of generative structural biology.
RFDiffusion~\citep{watson2023RFdiffusion} is a model that assists in designing protein structures for specific functions, such as enzymes. It is versatile in protein design and has been used to create therapeutic proteins, with some designs being confirmed in the laboratory.
% SMCDiff~\citep{trippe2022diffusion} is a model that generates scaffold structures for protein motifs. It predicts backbones and then builds scaffolds, yielding longer and more diverse outcomes compared to older methods.
ProteinSGM~\citep{lee2022proteinsgm} is a model that uses 2D matrices, which represent the distances and angles between protein parts, to create 3D protein structures for novel protein designs.
FoldingDiff~\citep{wu2022protein} is a model that generates protein sequences expected to fold into a specific structure. These sequences are verified with prediction tools, although they have not been experimentally confirmed yet.
Chroma~\citep{ingraham2023chroma} is a model designed for creating large proteins and protein complexes, considering various constraints like distances and symmetry. It transforms a collapsed polymer into protein backbone and sequence more quickly than older methods, thereby allowing for the efficient generation of large structures.

\subsection{Protein Inverse Folding}
The structure-based protein sequence design is typically formulated as a conditional sequence generation problem by deep generative modeling, wherein protein 3D structures are usually depicted as a \textit{k}-NN graph~\citep{ingraham2019generative}.
The protein graph establishes edge features between adjacent residues and encodes residue information as node features, modeled by graph neural networks (GNNs).
GraphTrans~\citep{ingraham2019generative} and GVP~\citep{jing2020gvp} utilizes the graph attention encoder and autoregressive decoder for protein design.
Recently, ProteinMPNN~\citep{dauparas2022proteinmpnn} and PiFold~\citep{gao2022pifold} introduce more complex protein features and expressive GNNs, resulting in significant improvements. 
Furthermore, in addition to the primary generative purpose, this task can also be used as a proxy for protein (structure-aware) representation learning~\citep{yang2022masked}.
A critical and significant challenge herein is the lack of sufficient protein structure data.
To this end, ESM-IF~\citep{hsu2022esmif} alleviate this issue with effective data augmentation by back-translation with AlphaFold 2~\cite{jumper2021AF2}.  , resulting in dramatic improvements. 
On the other hand, \citet{zheng2023structure} demonstrate how to efficiently steering large pretrained protein LMs into a structure-informed sequence generative models in a mask-predict generative manner, attaining state-of-the-art results on single-chain and complex protein benchmark.
Most recently, graph diffusion models have also been studied for inverse folding problem~\citep{yi2023gradeif}.


==> 041_experiment_bak.tex <==
\section{Experiments}
\label{sec:experiment}

We evaluate \method on various generative and understanding scenarios, including unconditional protein generation~(structure, sequence, and structure-sequence co-generation), and a variety of conditional tasks, such as folding, inverse folding and motif-scaffolding (\Secref{sec:cond motif}), and a series of protein predictive tasks (\Secref{sec:representation}).
% We show that \method is 





\subsection{Evaluation of Unconditional Protein Generation}
The goal of unconditional protein generation is to generate the 3D structure and 1D sequence of protein. 
Typically, this can be achieved with a cascade approach: first generating the structure, and then using a specialized inverse folding model to generate the sequence; or first sampling the sequence, followed with a folding model to obtain the structure. 
Additionally, the structure and sequence can also be generated simultaneously.
We assess \method on both cascaded generation paradigm and simultaneous way, resulting in \textit{unconditional structure generation}, \textit{unconditional sequence generation} and \textit{structure-sequence co-generation}.

We evaluate the generated proteins in terms of \textit{quality}, \textit{novelty} and \textit{diversity}, and the measurement of these metrics is introduced below.

\paragraph{Quality.} The quality encompasses two aspects: the \textit{designability} of structure and \textit{foldability} of sequence. 
Specifically, we measure designability on self-consistency, \ie, if there exists an amino acid sequence which can fold into the structure. We utilize ProteinMPNN~\citep{dauparas2022proteinmpnn} to sample amino acid sequences, then these sequences are folded into structures by state-of-the-art structure prediction model, \ie, ESMFold~\citep{lin2022esmfold}. 
And we calculate the \metric{TMscore} and \metric{RMSD} between \method generated structures and predicted structures, which we refer to \metric{sc-TMscore} and \metric{sc-RMSD}, respectively.
The higher \metric{sc-TMscore} or the lower \metric{sc-RMSD} means that the \method generated structure has higher designability.
On the other hand, the foldability of protein sequences reflects whether the sequence can be folded into a reasonable structures.
For each protein sequence, we utilize ESMFold~\citep{lin2022esmfold} to measure the foldability by the predicted local distance difference test (\metric{pLDDT}) score, which is considered a plausible structure if \metric{pLDDT} $>$ 70.

\paragraph{Novelty.} For each generated protein, we take the structure and compare the structural similarity against known structures in PDB with \metric{TMScore}. The highest \metric{TMscore} is used to assess the novelty, which we refer to \metric{pdb-TM}. A lower \metric{pdb-TM} indicates greater novelty.

\paragraph{Diversity.} We measure the diversity of generated protein by calculating the pairwise \metric{TMscore} between each pair of sampled protein structure and we refer to the highest \metric{TMscore} as \metric{inner-TM}, where a lower \metric{inner-TM} reveals that the generated proteins are more dissimilar.
Meanwhile, we also quantify the diversity by calculating the number of clusters utilizing FoldSeek~\citep{van2023foldseek} and dividing it by the total number of structures.




\input{tables/uncond_table}




\begin{figure*}[t]
    % \vspace{-1.5mm}
    \centering
    \includegraphics[width=\linewidth]{figures/uncond_main.pdf}
    \vspace{-3mm}
    \caption{{\sl Evaluation of unconditional generation.}
    % \textbf{(A)}: modeling, pre-training and unconditional generation; 
    % \textbf{(B)}: protein sequence representation for predictive tasks; 
    % \textbf{(C)}: conditional generation, including \textbf{(1)} sequence conditioning (\eg, motif-scaffolding), \textbf{(2)} cross-modal conditioning (\eg, inverse folding), and \textbf{(3)} plug-and-play controllable generation with discrete classifier guidance (\eg, secondary structure).
    }
    \label{fig:uncond_all}
    % \vspace{-2mm}
\end{figure*}



\subsubsection{Main Results}
\label{subsec:main results}
\Tabref{tab:uncond_main} and \Figref{fig:uncond_all} 
present the results of \method for unconditional protein generation.
We highlight our results in the following aspects:

\textbf{\method can generate highly designable and diverse structures unconditionally.} 
We sample 50 protein structures for each length of 100, 200, 300, 400 and 500.
Specifically, \method starts sampling structure tokens from 100\% noisy state, where reverse process iterates for 500 timesteps, and structure autoencoder reconstruct the 3D coordinates consequently.
\Tabref{tab:uncond_main} shows that \method achieves the highest \metric{sc-TMscore} compared to several strong baselines, closely approaching the native structures sampled from PDB.
\Figref{fig:uncond_all}A shows that \method is capable of sampling structures which possess high designability \textit{across various lengths}.
We can find that the distribution of \metric{sc-TMscore} is generally higher than $0.9$, where a structure is considered designable when \metric{sc-TMscore}$>0.5$~\citep{ingraham2023chroma}.

Interestingly, we find that the \metric{sc-RMSD}
of \method is not as impressive as \metric{sc-TMscore}.
Considering that \metric{RMSD} emphasizes local structural accuracy while \metric{TMscore} focuses on global structural integrity, we suggest that \method tends to generate globally reasonable structures that may possess local flexible conformations, resulting in a relatively high score of \metric{sc-RMSD}.
% \Figref{fig:ssp_all}D presents some \method sampled structures, and we find that despite the structures are not very globular and exhibit
% some non-idealized secondary structures and long loops, the \metric{sc-TMscore} is very high.
\Figref{fig:ssp_all}D presents some \method sampled structures, which are not very globular and exhibit
some non-idealized secondary structures and long loops.
We hypothesis this is due to the characteristic of the language modeling of discrete structure tokens.
During inference, we observe that \method randomly designates several positions as starting points, and then generates structure tokens in both directions from these positions, resultling in several substructures, which are concatenated together with loops at the end of inference.
Therefore, the final generated structure may contain several substructures linked with loops and not be as globular as structures generated by other backbone generation methods. 

% In addition, \Figref{fig:uncond_all}B reveals that the secondary structure distribution of \method generated structures is balanced and diverse~(\Figref{fig:uncond_all}), where the proportion of alpha-helix and beta-strand covers a variety of range. 
\Figref{fig:uncond_all}B presents the novelty of sampled proteins, and we find that \metric{pdb-TM} generally decreases with increasing length.
The long proteins, especially those with length 500, tend to be more novel.
And as shown in \Figref{fig:uncond_all}C, the number of structure clusters of each length is considerably high, which reveals \method is able to sample diverse proteins.
Notably, as protein length increases, the structure diversity grows while keeping designable, which means \method excels in handling long protein.

\textbf{\method is able to perform structure-sequence co-generation in a flexible way, where structure and sequence possess great consistency.
}
We show that \method can generate both structure and sequence of protein on its own in multiple ways, including simultaneous generation~(\textit{co-generation}), or cascaded workflow: first generating the structure then the sequence~(\textit{struct $\rightarrow$ seq}), and the reverse way~(\textit{seq $\rightarrow$ struct}), without the need of other folding or inverse folding models. During evaluation, we fold the generated sequence by ESMFold and calculate the \metric{TMscore} and \metric{RMSD} between the folded structure and the \method generated structure.

\Tabref{tab:uncond_main} reveals that the co-generated structures and sequences possess a high \metric{sc-TMscore}, exhibiting a high degree of consistency.
We suggest that this is because \method samples structure token and amino acid token at the same time, and the structure part and the sequence part actually serve as conditions for each other during generation process, which results in the consistency of structure and sequence.
Notably, the \metric{sc-TMscore} is close to the unconditionally generated structures and ProteinMPNN generated sequences, indicating that the co-genereted sequence has similar designability as ProteinMPNN.
Compared with MultiFlow~\citep{campbell2024generative}, \method achieves comparable co-generation quality, but we do not utilize the \textit{knowledge distillation} technique during training which is proved to significantly improve designability and diversity as noted in \citet{campbell2024generative}, indicating that \method may have substantial room for improvement.
Meanwhile, for the cascaded workflow~(struct $\rightarrow$ seq, seq $\rightarrow$ struct), the structure and sequence also demonstrate a strong level of consistency. 
Specifically, seq $\rightarrow$ struct leads to more diverse protein.
We conjecture this is due to \method inherits the sequence information from DPLM which is trained with immense natural sequences, resulting in more diverse sampled sequences, which are prompted to obtain diverse structure consequently.

% \Figref{fig:uncond_all}A shows that 
% We observe the co-generated 
% We show that \method can simultaneously generate both structure and sequence of a protein, without cascaded workflow.




\begin{figure*}[t]
    % \vspace{-1.5mm}
    \centering
    \includegraphics[width=\linewidth]{figures/ssp_main.pdf}
    \vspace{-3mm}
    \caption{{\sl Evaluation of secondary structure of generated proteins.}
    % \textbf{(A)}: modeling, pre-training and unconditional generation; 
    % \textbf{(B)}: protein sequence representation for predictive tasks; 
    % \textbf{(C)}: conditional generation, including \textbf{(1)} sequence conditioning (\eg, motif-scaffolding), \textbf{(2)} cross-modal conditioning (\eg, inverse folding), and \textbf{(3)} plug-and-play controllable generation with discrete classifier guidance (\eg, secondary structure).
    }
    \label{fig:ssp_all}
    % \vspace{-2mm}
\end{figure*}


\Figref{fig:uncond_all}H presents the co-generated structure and sequence.
The orange structure represents the \method generated structure, while grey for structure folded with \method generated sequence.
It can be seen that these two structures significantly overlap with each other, while keeping a high \metric{scTM} and low \metric{scRMSD}.
We suggest that this indicates: 
(1) the co-generated structure and sequence is consistent with each other, 
(2) the structure possesses high designability.
% (3) and the sequence exhibits a comparable level of designability to ProteinMPNN.

% with low \metric{sc-TMscore} score.
% The which indicates the structure and sequence co-generated reveal the same protein, with high designability.

% \Figref{fig:uncond_all}A shows that structure-sequence co-generation is more designable than unconditional structure generation, especially for long proteins. 
% Meanwhile, the protein structures sampled by co-generation is more diverse across various lengths.
% We suggest that \method benefits from multi-modal alignment, inheriting and transferring the evolutionary information from DPLM pretrained on the vast number of protein sequences into structure modeling. 
% Therefore, protein sequence can serve as pivot conditioning structure generation during co-generation, offering explicit evolutionary information and more possibilities from immense natural sequence space, resulting in more designable and diverse structure.

\textbf{\method is capable of sampling protein sequences with high structural plausibility across all lengths.}
We sample protein sequences of a set of lengths $[100, 200, ..., 900, 1000]$ in intervals of 100, for 500 iteration steps.
\Tabref{tab:uncond_main} and \Figref{fig:uncond_all}D shows that \method is capable of sampling protein sequences with high structural plausibility across all lengths.
Compared with DPLM, \method largely retains the original sequence generation capability, without serious catastrophic forgetting problem.
There is a slightly \metric{pLDDT} decrease in the length range of 600 to 1000 and probably due to limiting the training set's maximum length to 512. 
Consequently, \method does not encounter long proteins during training, resulting in reduced performance in sampling long proteins.



\subsubsection{Secondary Structure Analysis}

To further analyze the generated protein, we examine the secondary structure distribution, as illustrated in \Figref{fig:ssp_all}. The key findings are detailed below.

\paragraph{The secondary structure distribution of proteins sampled by \method is most similar to natural proteins.} 
We measure the proportions of each secondary structure, \ie, alpha helix, beta sheet and loop, in proteins sampled by different methods.
\Figref{fig:ssp_all}A illustrates that the structure-based diffusion models, such as RFDiffusion and MultiFlow, tend to generate proteins with significantly more helices and less sheets and loops than natural proteins in PDB.
For protein language models, such as ESM3 and \method, there is no obvious tendency to generate alpha helices.
However, the proteins sampled by ESM3 possess much more loop than PDB.
Compared with other methods, \method generates proteins with secondary structure proportions closest to those of PDB, demonstrating that the proteins sampled by \method best fit the natural distribution.

\Figref{fig:ssp_all}D visualize the generated proteins and natural proteins. 
Proteins sampled by MultiFlow contain a large amount of helices, and the proportion of alpha helices increases with protein length.
Moreover, proteins generated by MultiFlow are globular, compact, and exhibit nearly all idealized secondary structure elements.
In contrast, the \method generated proteins and natural proteins possess more balanced secondary structures with beta sheets and loops, instead of being dominated by the alpha helix. 
Furthermore, despite not being very globular or compact, proteins sampled by \method contain non-idealized and diverse local structural elements, including long loops and more beta strands, and looks more silimar to PDB.

On the other hand, as \Figref{fig:ssp_all}C shows, the proportion of loops has a significant impact on \metric{scRMSD}, with a higher loop proportion resulting in higher \metric{scRMSD} values.
% This is due to the loop region is very flexible and 
Considering that \method may sample proteins with long loops, the \metric{scRMSD} metric will be relatively high, which is consistent with \Tabref{tab:uncond_main}.
We also plot the secondary structure ternary graph of each protein in \Figref{fig:ssp_all} D. 
Compared with natural proteins, the points of MultiFlow are clearly concentrated in regions with a higher number of helix and lower number of loops, while points of \method can largely cover the natural proteins.
However, we find that \method rarely samples proteins composed only of loops and sheets with few helices, which exist in natural proteins.

\paragraph{The learned structure tokens inherently contain connections with secondary structures.}
We explore the information contained in learned structure tokens and find a correlation with secondary structures.
Specifically, we collect structures sampled by \method and analyze the statistical patterns of structure tokens and secondary structures at each position.
We plot the simplex of the secondary structure for each structure token in \Figref{fig:ssp_all}B.
The bright areas represent high density, which means these areas contains many structure tokens, whereas the opposite indicates low density.
The closer the structure token is to the vertices of the ternary, the more deterministically it corresponds to a specific secondary structure.

It can be seen that the vast majority of points are concentrated in the vertices corresponding to the alpha helix and beta sheet and a few points to the loop, while the density of points in the center of the triangle is low, which demonstrates that most of the learned structure tokens have a clear correspondence with a secondary structure.
Meanwhile, we also find that some structure tokens distribute between the alpha helix and beta sheet or loop and beta sheet, illustrating that there structure tokens are correlated with two secondary structures, and determine the correspondence according to the context.



\input{tables/ablation}

\subsubsection{Ablation Study}
During \method training, we initialize model parameters from the sequence-based pretrained model to transfer evolutionary information and augment the training data using high quality alphafold predicted structures~(SwissProt, approximately 200K data) in addition to PDB. 
We examine the effect of both sequence pretraining and training data augmentation on the unconditional protein generation.

\Tabref{tab:ablation} demonstrates that \textit{sequence pretraining and data augmentation can significantly improve the designability and diversity}, especially in the long protein sampling~(length exceeding 300).
We hypothetis that the limited number of long proteins in the PDB results in insufficient training.
In contrast, the sequence pretraining, which incorporates evolutionary information, plays a crucial role and can be transferred in the protein structure modeling, thereby enhancing protein generation quality. Additionally, the evolutionary information from the large protein sequence space can also improve the sampling diversity.
On the other hand, directly increasing the number of training data can also improve designability, but it falls short in enhancing diversity compared to sequence pretraining.
Combining the two techniques can achieve the best overall results, so we take them both as our training strategy.

% \paragraph{\method } 
% \paragraph{On designability.} 
% % \ul{DPLM-2 is capable of sampling structures which possess high designability.}
% We evaluate the \method ability of sampling designable structures, 
%  for structures \method generates, we 



% \paragraph{Case study.}
% \Figref{fig:uncond_all}E shows protein structure sampled by \method, while more cases are presented in Appendix.
% We find that \method can sample complex structures containing rich helices and sheets while possess high \metric{sc-TMscore}.


% \subsubsection{Unconditional Structure-sequence Co-generation}
% \label{sec:uncond co-generation}

% We mainly focus on the structure part of co-generation, and the sampled protein length and iteration timesteps are the same as unconditional structure generation (\Secref{sec:uncond struct}).




\subsection{Folding}
\label{sec:cond folding}

We investigate the conditional generation ability of \method, and we mainly focus on two tasks: folding and inverse folding.

\input{tables/folding}
% \paragraph{Folding}
% \phantomsection
% \label{sec:cond folding}
The goal of folding is to find the 3D structure of the given amino acid sequence.
\method takes single amino acid sequence concatenated by noisy structure token as input, without need for multiple sequence alignment.
For higher accuracy, the decoding strategy of \method is \metric{argmax}, \ie, pick the token with the highest probability instead of random sampling, and iterate for 100 steps.
We split the PDB by clusters and divide proteins of 50 clusters to test set.
Meanwhile, we also assess \method on the common folding test set CAMEO 2022.
We utilize \metric{RMSD} and \metric{TMscore} between predicted and ground truth structure for evaluation.


\textit{\method is capable of producing highly accurate structure predictions for specified amino acid sequences.}
% We evaluate the \method \ie, zero-shot generation, and additional supervised funetuning~(SFT training). 
\Tabref{tab:folding} indicates that \method can perform folding without additional training, \ie, in a zero-shot way, and even better after SFT training.
Overall, \method can outperform or on par with the strong baselines, while achieving close performance with ESMFold.
We suggest that \method benefits from the evolutionary information inherited from DPLM pretrained on the vast number of protein sequences, which can be transferred and leveraged into structure modeling. 
Furthermore, We observe that \method with larger model scales can attain better results than smaller ones, revealing the scaling law~\citep{kaplan2020scaling}.
Interestingly, we discover a scaling pattern that the SFT training performance of \method is very close to the zero-shot performance of larger scale, for example, \method 150M with SFT training performs very similar to \method 650M.
This pattern indicates that we can conveniently predict the larger model performance according to the SFT performance of current one.

\subsection{Inverse Folding}
\label{sec:cond inversefolding}
% \label{sec:cond inversefolding}

\input{tables/invfold}
The goal of inverse folding is to find an amino acid sequence that can fold to a given protein backbone structure.
During inference, \method picks the token with highest probability with 100 iteration steps.
We evaluate \method on the clustered test-out dataset from PDB and CAMEO dataset as same to the folding evaluation.
For evaluation metric, we employ amino acid recovery (AAR) for sequence evaluation, and we also assess the structure by first predict the structure of the generated sequence using ESMFold, and then compute the \metric{pLDDT} score and self-consistency TM-score (\metric{scTM}) between the predicted structure and the input structure.

\textit{\method can generate reasonable sequences which can be folded into the given structures.} 
\Tabref{tab:folding} presents that \method can outperform or be on par with other co-generation models~(MultiFlow, ESM3).
As the model size increases, the performance in terms of sequence recovery~(\metric{AAR}) and structural consistency~(\metric{scTM}) improves, revealing the same scaling law observed in the folding task.
We suggest that multi-modal training effectively aligns the structure and sequence into the same space.
When given structure information, \method can yield the corresponding sequence without additional training.



% \input{tables/motif_table}


\subsection{Motif-scaffolding}
\label{sec:cond motif}


\begin{figure*}[h]
    \centering
    % \vspace{-1mm}
    \includegraphics[width=\linewidth]{figures/motif_main.pdf}
    \vspace{-5mm}
    \caption{{\sl Evaluation of motif-scaffolding.}
    \textbf{(A)} comparison regarding overall success rate and number of solved problems;
    \textbf{(B)} comparison between sequence-only approaches (\method \vs RFDffusion);  
    \textbf{(C)} comparison between structure-aware approaches (structure-conditioned \method \vs ESM3); and
    % \textbf{(D)} comparison between sequence-only \vs structure-conditioned \method.
    % \textbf{(E)} case study for three problems.
    % 
    }
    \label{fig:motif_main}
    % \vspace{-2mm}
\end{figure*}


The objective of motif-scaffolding is to generate a suitable scaffold to preserve the structure of the given motif and maintain its original function.
% We follow the experimental setting of \citet{wang2024diffusion}, 
We follow the experimental setting of \citet{yim2024improved},
for each motif case, we 
(1) first determine the length of scaffold, and then
(2) keep the motif segment unchanged and sample the scaffold part conditioned on the motif.
The scaffold length is sampled from a range provided by \citet{yim2024improved}, and when there are multiple motifs, the order of motif segments is consistent with \citet{yim2024improved}.
We provide the 3D structure and sequence of motif as input of \method.
The generated proteins are assessed based on two criteria:
(1) overall quality, which is successful when \metric{pLDDT} $> 70$ or \metric{scTM} $> 0.8$, and
(2) motif part consistency, which is deemed successful when the \metric{RMSD} between the predicted motif structure and the ground truth, which we refer to as \metric{motif-RMSD}, is less than $1\AA$. 
% referred to as \metric{motif-RMSD} .
A scaffold is considered successful if it satisfies both criteria.
Overall, we examine 24 motif-scaffolding problems, and for each problem, we sample 100 sequences and then calculate the success rate according to the above criterion.

We evaluate \method using sequence-based, structure-based, and co-generation methods.
The evaluation of overall quality varies across methods.
(1) For sequence-based method, we only take the generated sequence and utilize ESMFold to obtain the predicted structure, and the \metric{pLDDT} score provided by ESMFold is used to assess overall quality.
(2) For structure-based method, we only take the generated structure, and then leverage ProteinMPNN to predict the sequence, followed by ESMFold to predict the structure, where overall quality is assessed by \metric{scTM}.
(3) For co-generation method, we take both the generated structure and sequence, and predict structure given generated sequence with ESMFold, where \metric{scTM} 
 is calculated between generated structure and ESMFold predicted structure to evaluate overall quality.
Considering that the ground truth motif structure is given, we only utilize the ESMFold predicted structure to calculate \metric{motif-RMSD}.

% During sampling and evaluation, we employ different ways to compare with the corresponding methods.
% (1) For sequence-centric method, such as DPLM~\citep{wang2024diffusion} or 
% EvoDiff~\citep{alamdari2023protein}, we utilize ESMFold~\citep{lin2022esmfold} to predict the structure of generated sequence
% , and utilize the co-generation paradigm described in \Secref{sec:inference} to sample the structure and sequence of the whole protein simultaneously.
% We take the structure generated by \method for assessment. 

% while for ESM3~\citep{esm3}, we follow the evaluation pipeline in their paper, which first generates the sequence and then reconstruct the structure conditioning on the sequence.
% A scaffold is considered successful 


\Figref{fig:motif_main} reveals that \method is capable of generate reasonable scaffolds for the given functional motifs.
We observe that \method outperforms sequence-centric method in most cases, solving more motif problem and achieving higher average success rate, indicating the importance of multi-modal modeling that being able to utilize more comprehensive protein conditions.
Compared with ESM3, \method achieve a comparable performance in the same number of solved problems and slightly higher success rate. 
Specifically, we find that \method shows better results in 8 cases, while ESM3 outperforms in 6 cases.
Considering that \method uses significantly less training overhead than ESM3, this underscores the importance of evolutionary information in pre-trained protein language models and the effectiveness of transfer learning.



\subsection{Evaluation of Protein Representation Learning}
\label{sec:representation}


==> 050_conclusion.tex <==
\section{Discussions}
\label{sec:conclusion}

In this paper, we introduce diffusion protein LM (\method), a versatile protein LM that is capable of both protein sequence generation and representation learning. 
We further develop several conditioning strategies for various needs of conditional generation, including sequence conditioning, cross-modal conditioning, and programmable generation with plug-and-play discrete classifier guidance.

Despite these promising results, there remain several limitations and future work directions deserving to be explored. 


\begin{compactitem}

\item[(i)] \textit{Exploring \method's conditional generation for wider applications.}
We can further extend the cross-modal conditioning strategy of \method to more diverse modalities as conditioners, including MSA-conditioned homologous sequence generation, small molecule-conditioned binder design for ligands, antigen-conditioned antibody CDR design, among others. 
Also, the inclusion of demonstrations featuring plug-and-play classifier-guided controllable generation is essential for more scenarios toward diverse user preferences, \eg, structural symmetry, superfamily, binding affinity, thermostability, fluorescence, and beyond.

 
\item[(ii)] \textit{\method can further benefit from best practices of cutting-edge technical advancement in the vastness of large language models (LLMs).}
For example, \textbf{(1)} long context extension~\citep{chen2023extending} can rapidly adapt \method to handle very long proteins beyond its training length limit, and offering potential for modeling exceptionally long biological sequences such as DNAs and RNAs, unifying and deciphering the languages associated with the central dogma of life; 
\textbf{(2)} fine-tuning \method with human feedback or even wet-lab experimental feedback, leveraging reinforcement learning~\citep[RL;][]{ouyang2022instructgpt}, direct preference optimization~\citep[DPO;][]{rafailov2024dpo}, and self-play fine-tuning~\citep{chen2024spin};
\textbf{(3)} eliciting instruction-following and in-context learning~\citep{wei2022emergent} analogs for protein LMs can also be a promising direction would fully harness \method's learned knowledge.

\item[(iii)] \textit{It is imperative to integrate protein structure modeling into \method.}
The advance of protein structure modeling manifest tremendous success, including AlphaFold~\citep{jumper2021AF2}, ESMFold~\citep{lin2022esmfold} for structure prediction, RFDIffusion~\citep{watson2023RFdiffusion}, Chroma~\citep{ingraham2023chroma} for structure design, and even full-atom molecular modeling, \eg, the latest generation of AlphaFold~\citep{deepmind2023AF3} and RF-AA~\citep{krishna2023RFAA}. 
Developing a universal protein language model with the next-generation \method, which accounts for both sequence and structure, is a particularly promising avenue.

\end{compactitem}


We leave these exciting directions as future work.

==> tables/cath.tex <==
\begin{table}[t!]
   \centering
   \small
   \setlength{\tabcolsep}{2pt}
   \vspace{-2mm}
   \caption{{\sl Performance comparison between \method and different baseline approaches on CATH 4.2 and CATH 4.3 datasets.}
   {\method's results are obtained by \texttt{argmax} decoding (\ie, no sampling).}
   $\dagger$: benchmarked results are quoted from \citet{gao2022pifold}.
   }
   % \vspace{1.5pt}
   \label{tab:results_cath}

   \resizebox{\linewidth}{!}{%
   \begin{tabular}{llrccc}
   \toprule
   & \multirow{2}{*}{ Models} 
   & \multirow{2}{*}{ Trainable} 
   & \multirow{2}{*}{\metric{AAR}} 
   & \multicolumn{2}{c}{ struct. eval.} \\
    \cmidrule[0.3pt](lr){5-6} & & Params. & & \metric{scTM}  & \metric{pLDDT} \\
   \midrule
   % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

   %%%%%%%%%%%%%%%%%%%%%%%%%%
   \multirowcell{7}{\rotatebox[origin=c]{90}{CATH 4.2}}
   & $^\dagger$StructTrans~\smallcitep{ingraham2019generative}                     & 1.6M/1.6M  & 35.82&   -   & - \\
   % & GCA&  7.09&  7.49  &  6.05  & 32.62 & 31.10 & 37.64 \\
   & $^\dagger$GVP~\smallcitep{jing2020gvp}                                       & 1.0M/1.0M  &  39.47 &   - & -  \\
   % & AlphaDesign &  7.32  & 7.63 &  6.30 &  34.16  & 32.66  &  41.31   \\
   & $^\dagger$ProteinMPNN~\smallcitep{dauparas2022proteinmpnn}                   & 1.9M/1.9M  &  45.96 &  -  & -    \\
   & PiFold~\smallcitep{gao2022pifold} \                                        & 6.6M/6.6M  &  {51.66} &   {-} &{-}  \\ 
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  & ProteinMPNN + CMLM                                                 & 1.9M/1.9M  &48.62     & 0.87 & 74.07 \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  &\chl 7.02 & \chl 6.67 & \chl 4.63   & \chl 35.71  & \chl 38.61 & \chl 53.26 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 7.33 & \chl 6.83 & \chl 4.63 & \chl \textbf{36.47} & \chl \textbf{40.91} & \chl \textbf{54.62} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  &50.22  &- &-   \\ 

  &  \textsc{LM-Design} (\textit{w/} ProtMPNN encoder)              &  5.0M/650M   &  {54.41} &  0.88 &  77.07 \\
  & \chl \method (\textit{w/} ProtMPNN encoder)              & \chl 5.0M/650M   & \chl \textbf{54.54} & \chl 0.88 & \chl \textbf{77.12} \\
  \midrule
  % \cmidrule[0.5pt](lr){2-8}

  %%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirowcell{6}{\rotatebox[origin=c]{90}{CATH 4.3}}
  & PiFold~\smallcitep{gao2022pifold} & 6.6M/6.6M    &  {51.66} & - & - \\ 
  & GVP-Transformer~\citep{hsu2022esmif}                                 & 142M/142M  &  51.60 &   - & -  \\
  &  \textsc{LM-Design} (\textit{w/} GVP-Trans encoder)          &  6.3M/650M  & 56.49 &  0.85 & 74.89  \\

  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  % & ProteinMPNN + CMLM                                                  & 1.9M/1.9M  & 6.31 &6.32  &4.85     & 40.30 & 39.02 &  48.25  \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.96 &\chl 5.85 &\chl 4.48   & \chl 44.12  & \chl 44.05 &\chl 54.05 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.94 & \chl 5.80 & \chl 4.20 & \chl 45.65 & \chl \textbf{46.15} & \chl 55.92 \\
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{5.88} & \chl \textbf{5.66} & \chl \textbf{4.19} & \chl \textbf{45.71} & \chl \textbf{46.15} & \chl \textbf{56.38} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 5.88& 5.55 & 4.47  & 42.86 &43.69& 50.68    \\ 
  & \chl \method-150M (\textit{w/} GVPTrans encoder)                                               & \chl 3.1M/{150M}   &\chl {53.27}   & \chl {0.85}  &\chl \textbf{75.31}  \\ 
  & \chl \method-650M (\textit{w/} GVPTrans encoder)                                               & \chl 6.3M/{650M}   &\chl {56.61}   & \chl {0.86}  &\chl {76.78}  \\ 
   & \chl \method-3B (\textit{w/} GVPTrans encoder)                                               & \chl 68.2M/{3.0B}   &\chl \textbf{59.44}   & \chl \textbf{0.86}  &\chl \textbf{77.12}  \\ 
\bottomrule
\end{tabular}
}
   \vspace{8pt}
\end{table}


==> tables/folding_old.tex <==
\begin{table*}[t!]
   \centering
   \small
   \setlength{\tabcolsep}{2pt}
   \vspace{-2mm}
   \caption{{\sl Structure prediction performance comparison between \method and different baseline approaches on CAMEO 2022 datasets.}
   {\method's results are obtained by \texttt{argmax} decoding (\ie, no sampling).}
   $\dagger$: benchmarked results are quoted from \citet{haiyan2023diffusion}.
   }
   % \vspace{1.5pt}
   \label{tab:folding}

   \resizebox{0.9\linewidth}{!}{%
   \begin{tabular}{llcccccccc}
   \toprule
    & \multirow{2}{*}{ Models} 
    & \multicolumn{2}{c}{CAMEO 2022} 
    & \multicolumn{2}{c}{CASP} 
    & \multicolumn{2}{c}{PDB-cluster}
    & \multicolumn{2}{c}{PDB-date} \\
    \cmidrule[0.3pt](lr){3-4} \cmidrule[0.3pt](lr){5-6}
    \cmidrule[0.3pt](lr){7-8} \cmidrule[0.3pt](lr){9-10}& & {\metric{RMSD}} & {\metric{TMscore}} & {\metric{RMSD}} & {\metric{TMscore}} & {\metric{RMSD}} & {\metric{TMscore}} &{\metric{RMSD}} & {\metric{TMscore}} \\
   \midrule
   % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

   %%%%%%%%%%%%%%%%%%%%%%%%%%
   \multirowcell{12}{\rotatebox[origin=c]{90}{Folding}}
   & $^\dagger$ESMFold~\smallcitep{lin2022esmfold}
   & 3.99/2.03  &  0.85/0.93    \\
   % & $^\dagger$OmegaFold~\smallcitep{wu2022high}                                 & 5.26/2.62  &  0.80/0.89   \\
   % & $^\dagger$EigenFold~\smallcitep{jing2023eigenfold}                   
   % & 7.37/3.50  &  0.75/0.84   \\
   & $^\dagger$PVQD~\smallcitep{haiyan2023diffusion}                             & 4.08/1.95  &  0.81/0.88   \\
   & MultiFlow~\smallcitep{campbell2024generative}
   & TODO  &  TODO   \\
   & ESM3
   & TODO  &  TODO   \\
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-4}  
  & \chl \method~(150M)
  & \chl 9.22/7.64  & \chl 0.75/0.81  
  & & 
  & \chl 6.99/3.96  & \chl 0.78/0.85
  & & \\ 
  
  & \chl \qquad \textit{w/} SFT training
  & \chl 7.66/4.37  & \chl 0.80/0.86    
  & & 
  & \chl 4.97/2.87  & \chl 0.84/0.88
  & & \\
  
  & \chl \method~(650M)   
  & \chl 7.37/4.89  & \chl 0.79/0.86   
  & & 
  & \chl 4.72/2.55  & \chl 0.84/0.88
  & & \\ 
  
  & \chl \qquad \textit{w/} SFT training
  & \chl 6.21/3.78  & \chl 0.84/0.89    
  & & 
  & \chl 3.66/2.30  & \chl 0.87/0.91 
  & & \\
  
  & \chl \method~(3B)     
  & \chl 6.34/3.65  & \chl 0.83/0.89   
  & & 
  & \chl 4.00/2.28  & \chl 0.87/0.92
  & & \\ 
  
  & \chl \qquad \textit{w/} SFT training
  & \chl 5.71/3.23  & \chl 0.85/0.90    
  & & 
  & \chl 3.29/2.38  & \chl 0.88/0.92  
  & & \\

  \midrule
  %\cmidrule[0.5pt](lr){2-8}
  & 
  & \metric{AAR} & \metric{scTM} 
  & \metric{AAR} & \metric{scTM} 
  & \metric{AAR} & \metric{scTM} 
  & \metric{AAR} & \metric{scTM} \\
  \midrule
  %%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirowcell{5}{\rotatebox[origin=c]{90}{Inverse Folding}}
  & {MultiFlow}~\smallcitep{campbell2024generative}
  &  TODO  & TODO   \\
  & ESM3
   & TODO  &  TODO   \\

  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-10}  
  & \chl \method~(150M)
  & \chl 45.22/46.12  & \chl 0.87/0.93
  & & 
  & \chl 50.76/49.86  & \chl 0.90/0.95
  & \chl & \chl 0.89/0.95 \\ 
  
  & \chl \method~(650M)   
  & \chl 49.01/50.10  & \chl 0.88/0.93
  & & 
  & \chl 53.37/52.03  & \chl 0.92/0.96
  & \chl  & \chl 0.91/0.96 \\ 
  
  & \chl \method~(3B)     
  & \chl 52.36/53.72  & \chl 0.89/0.95
  & & 
  & \chl 57.90/56.87  & \chl 0.92/0.97
  & \chl & \chl 0.92/0.96 \\ 
  
\bottomrule
\end{tabular}
}
   \vspace{8pt}
\end{table*}


==> tables/inverse_folding.tex <==
% \begin{table*}[t]
%    \centering
%    \small
%    % \setlength{\tabcolsep}{5pt}
%    \vspace{-2.5mm}
%    \caption{{\sl Performance comparison between \method and different baseline approaches on CATH 4.2 and CATH 4.3 datasets.} {\method's results are obtained by 5-cycle iterative refinement with \texttt{argmax} operator (\ie, no sampling).}
%    $\dagger$: benchmarked results are quoted from \citet{gao2022pifold}.
%    $\ddagger$: ``Single-chain'' in \citet{hsu2022esmif} is defined differently. ESM-1b 650M is used as the default \pLM.}
%    \vspace{1.5pt}
%    \label{tab:inverse_folding}

%    \resizebox{\linewidth}{!}{%
%    \begin{tabular}{llrccc}
%    \toprule
%    & \multirow{2}{*}{\bf Models} 
%    & \multirow{2}{*}{\bf Trainable/Total} 
%    & \multicolumn{1}{c}{\bf Sequence Metric ($\uparrow$)} 
%    & \multicolumn{2}{c}{\bf Structure Metric (\%, $\uparrow$)} \\
%    \cmidrule[0.3pt](lr){4} \cmidrule[0.3pt](lr){5-6}
%    & & \bf Params. & AAR   & scTMscore  & pLDDT \\
%    \midrule
%    % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

%    %%%%%%%%%%%%%%%%%%%%%%%%%%
%    \multirowcell{10}{\rotatebox[origin=c]{90}{CATH 4.2}}
%    & $^\dagger$Structured Transformer~\smallcitep{ingraham2019generative}                     & 1.56M/1.56M  & 8.39  & 8.83 & 6.63 \\
%    % & GCA&  7.09&  7.49  &  6.05  & 32.62 & 31.10 & 37.64 \\
%    & $^\dagger$GVP~\smallcitep{jing2020gvp}                                       & 1.0M/1.0M  & 7.23  &   7.84 &  5.36  \\
%    % & AlphaDesign &  7.32  & 7.63 &  6.30 &  34.16  & 32.66  &  41.31   \\
%    & $^\dagger$ProteinMPNN~\smallcitep{dauparas2022proteinmpnn}                   & 1.9M/1.9M  & 6.21  &   6.68  &  4.61  \\
%    & PiFold~\smallcitep{gao2022pifold} \                                & 6.6M/6.6M  & {6.04}  &   {6.31}  &  {4.55}  \\ 
%   %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
%   \cmidrule[0.5pt](lr){2-9}
%   & ProteinMPNN + CMLM [ProtMPNN-CMLM]                                                 & 1.9M/1.9M  &7.16 &7.25  & 5.03     \\ 
%   & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  &\chl 7.02 & \chl 6.67 & \chl 4.63    \\ 
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 7.33 & \chl 6.83 & \chl 4.63  \\
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{7.01} & \chl \textbf{6.58} & \chl \textbf{4.41} \\
%   \cmidrule[0.2pt](lr){2-9}
%   & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 6.94 &6.82  &4.69   \\ 
%   & \chl \method (PiFold)                                               & \chl 11.9M/664M (\textbf{1.7\%})  & \chl \textbf{6.77} & \chl \textbf{6.46}   & \chl \textbf{4.52}   \\ 
%   \midrule
%   % \cmidrule[0.5pt](lr){2-8}

%   %%%%%%%%%%%%%%%%%%%%%%%%%%
%   \multirowcell{10}{\rotatebox[origin=c]{90}{CATH 4.3}}
%   & GVP-large~\citep{hsu2022esmif}                                      & 21M/21M  &  7.68  & $^\ddagger$6.12~~ &  6.17   \\
%   & GVP-Transformer~\citep{hsu2022esmif}                                 & 142M/142M  &   8.18 & $^\ddagger$6.33~~ &  6.44  \\
%   & ~~~~+1.2M AF2 predicted data~\smallcitep{hsu2022esmif}              & 142M/142M  &   6.05 & $^\ddagger$4.00~~ &  4.01 \\
%   & \chl \method (pretrained GVP-TransEncoder: \textit{freeze})          & \chl 6.3M/800M (\textbf{0.8\%})  & \chl 6.61 & \chl 7.64 & \chl \textbf{3.92} \\
%   % & PiFold~\smallcitep{gao2022pifold} \   &  {6.04}  &   {6.31}  &  {4.55} &   {39.84} &{38.53} &  {51.66} \\ 
%   %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
%   \cmidrule[0.5pt](lr){2-9}
%   & ProteinMPNN + CMLM                                                  & 1.9M/1.9M  & 6.31 &6.32  &4.85      \\ 
%   & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.96 &\chl 5.85 &\chl 4.48    \\ 
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.94 & \chl 5.80 & \chl 4.20  \\
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{5.88} & \chl \textbf{5.66} & \chl \textbf{4.19}  \\
%   \cmidrule[0.2pt](lr){2-9}
%   & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 5.88& 5.55 & 4.47   \\ 
%   & \chl \method (PiFold)                                               & \chl 11.9M/664M (\textbf{1.7\%})  &\chl \textbf{5.66} &\chl \textbf{5.52}  &\chl 4.01  \\ 
  
%    \bottomrule
%    \end{tabular}
%    }
%    % \vspace{-8pt}
% \end{table*}



=========================
% \begin{table*}[]
% \begin{tabular}{lllll}
% \hline
%                             & Params & AAR & scTMscore & pLDDT          \\ \hline
% PiFold                      & 6.6M                           & 50.68                       & TODO                              & TODO           \\
% GRADE-IF                    & -                              & TODO                        & TODO                              & TODO           \\
%                             & 150m                           & 53.08                       & 0.84                              & 74.40          \\
% \multirow{-2}{*}{LM-DESIGN} & 650m                           & \textbf{56.69}              & 0.85                              & 74.89          \\
%                             & 150m                           & \textbf{53.27}              & 0.84                              & 73.84          \\
% \multirow{-2}{*}{\chl DIFF-LM}   & 650m                           & 56.36                       & \textbf{0.8575}                   & \textbf{76.94} \\ \hline
% \end{tabular}
% \end{table*}

==> tables/motif_omegafold.tex <==
\begin{table}[t!]
   \centering
   \small
   \setlength{\tabcolsep}{2pt}
   \vspace{-3mm}
   \caption{{\sl Performance comparison between \method and different baseline approaches on CATH 4.2 and CATH 4.3 datasets.}
   {\method's results are obtained by \texttt{argmax} decoding (\ie, no sampling).}
   $\dagger$: benchmarked results are quoted from \citet{gao2022pifold}.
   }
   % \vspace{1.5pt}
   \label{tab:results_cath}

   \resizebox{\linewidth}{!}{%
   \begin{tabular}{llrccc}
   \toprule
   & \multirow{2}{*}{ Models} 
   & \multirow{2}{*}{ Trainable} 
   & \multirow{2}{*}{\metric{AAR}} 
   & \multicolumn{2}{c}{\bf struct. eval.} \\
    \cmidrule[0.3pt](lr){5-6} & & \bf Params. & & \metric{scTM}  & \metric{pLDDT} \\
   \midrule
   % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

   %%%%%%%%%%%%%%%%%%%%%%%%%%
   \multirowcell{7}{\rotatebox[origin=c]{90}{CATH 4.2}}
   & $^\dagger$StructTrans~\smallcitep{ingraham2019generative}                     & 1.6M/1.6M  & 35.82&   -   & - \\
   % & GCA&  7.09&  7.49  &  6.05  & 32.62 & 31.10 & 37.64 \\
   & $^\dagger$GVP~\smallcitep{jing2020gvp}                                       & 1.0M/1.0M  &  39.47 &   - & -  \\
   % & AlphaDesign &  7.32  & 7.63 &  6.30 &  34.16  & 32.66  &  41.31   \\
   & $^\dagger$ProteinMPNN~\smallcitep{dauparas2022proteinmpnn}                   & 1.9M/1.9M  &  45.96 &  -  & -    \\
   & PiFold~\smallcitep{gao2022pifold} \                                        & 6.6M/6.6M  &  {51.66} &   {-} &{-}  \\ 
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  & ProteinMPNN + CMLM                                                 & 1.9M/1.9M  &48.62     & - & - \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  &\chl 7.02 & \chl 6.67 & \chl 4.63   & \chl 35.71  & \chl 38.61 & \chl 53.26 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 7.33 & \chl 6.83 & \chl 4.63 & \chl \textbf{36.47} & \chl \textbf{40.91} & \chl \textbf{54.62} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  &50.22  &- &-   \\ 

  &  \textsc{LM-Design} (\textit{w/} ProtMPNN encoder)              &  5.0M/659M   &  {54.41} &  0.88 &  77.07 \\
  & \chl \method (\textit{w/} ProtMPNN encoder)              & \chl 5.0M/659M   & \chl \textbf{54.54} & \chl 0.88 & \chl \textbf{77.12} \\
  \midrule
  % \cmidrule[0.5pt](lr){2-8}

  %%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirowcell{4}{\rotatebox[origin=c]{90}{CATH 4.3}}
  & PiFold~\smallcitep{gao2022pifold} & 6.6M/6.6M    &  {51.66} & - & - \\ 
  & GVP-Transformer~\citep{hsu2022esmif}                                 & 142M/142M  &  51.60 &   - & -  \\
  &  \textsc{LM-Design} (\textit{w/} GVP-Trans encoder)          &  3.1M/302M  & 53.08 &  0.84 & 74.40  \\
  &  \textsc{LM-Design} (\textit{w/} GVP-Trans encoder)          &  6.3M/800M  & 56.49 &  0.85 & 74.89  \\
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  % & ProteinMPNN + CMLM                                                  & 1.9M/1.9M  & 6.31 &6.32  &4.85     & 40.30 & 39.02 &  48.25  \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.96 &\chl 5.85 &\chl 4.48   & \chl 44.12  & \chl 44.05 &\chl 54.05 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.94 & \chl 5.80 & \chl 4.20 & \chl 45.65 & \chl \textbf{46.15} & \chl 55.92 \\
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{5.88} & \chl \textbf{5.66} & \chl \textbf{4.19} & \chl \textbf{45.71} & \chl \textbf{46.15} & \chl \textbf{56.38} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 5.88& 5.55 & 4.47  & 42.86 &43.69& 50.68    \\ 
  & \chl \method (\textit{w/} GVP-Trans encoder)                                               & \chl 3.1M/302M   &\chl \textbf{53.27}   & \chl \textbf{0.85}  &\chl \textbf{75.31}  \\ 
  & \chl \method (\textit{w/} GVP-Trans encoder)                                               & \chl 6.3M/800M   &\chl \textbf{56.61}   & \chl \textbf{0.86}  &\chl \textbf{76.78}  \\ 
  
\bottomrule
\end{tabular}
}
   % \vspace{-8pt}
\end{table}


==> tables/motif_success.tex <==
\begin{table}[t]
\centering
\vspace{-1.5mm}
% \setlength{\tabcolsep}{2.5pt}
\caption{Results of the success rate of each problem, the number of the solved problems and the average success rate across 17 motif-scaffolding problems. Here we follow previous work to use OmegaFold as the folding model.}
\label{tab:motif_success}
\vspace{1.5pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{{seq-only}} & \multicolumn{2}{c}{{struct-cond.}} \\ 
\cmidrule[0.5pt](lr){2-3}  \cmidrule[0.5pt](lr){4-5}
                  & EvoDiff        & DPLM                 & RFDiffusion        & DPLM   \\
\midrule
1bcf              & 0.39           & \textbf{0.99}        & 1.00                 & 1.00                    \\
1prw              & 0.87           & \textbf{0.96}        & 0.08               & \textbf{0.99}        \\
1qjg              & 0.00              & 0.00                    & 0.00                  & 0.00                    \\
1ycr              & 0.13           & \textbf{0.52}        & 0.74               & \textbf{0.78}        \\
2kl8              & 0.03              & \textbf{0.05}        & 0.88               & 0.05                 \\
3ixt              & 0.26           & 0.20                  & 0.25               & \textbf{0.33}        \\
4jhw              & 0.00              & 0.00                    & 0.00                  & 0.00                    \\
4zyp              & 0.00              & \textbf{0.01}        & 0.40                & 0.01                 \\
5ius              & 0.00              & \textbf{0.10}         & 0.02               & \textbf{0.10}         \\
5tpn              & 0.00              & 0.00                    & 0.61               & 0.00                    \\
5trv              & 0.00              & 0.00                    & 0.22               & 0.00                    \\
5wn9              & 0.00              & \textbf{0.01}        & 0.00                  & \textbf{0.01}        \\
5yui              & 0.06           & \textbf{0.42}        & 0.00                  & \textbf{0.63}        \\
6e6r              & 0.16           & \textbf{0.84}        & 0.71               & \textbf{0.84}        \\
6exz              & 0.00              & \textbf{0.01}        & 0.42               & 0.01                 \\
6vw1              & 0.00           & 0.00                    & 0.69               & 0.00                    \\
7mrx              & 0.00              & \textbf{0.59}        & 0.07               & \textbf{0.59}        \\ 
\midrule
pass rate         & 7/17           & \textbf{12/27}       & 13/17              & 12/17                \\
avg. success rate & 0.09           & \textbf{0.27}        & 0.36               & 0.31                 \\ 
\bottomrule
\end{tabular}
}
\vspace{4mm}
\end{table}

==> tables/motif_table.tex <==
\begin{table}[t]
\centering
\vspace{-1.5mm}
% \setlength{\tabcolsep}{2.5pt}
\caption{Motif-scaffolding results evaluated by ESMFold. }
\label{tab:motif_main}
\vspace{1.5pt}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{\textbf{Seq-only}} & \multicolumn{1}{c}{Struct-cond.} \\ 
% \cmidrule[0.5pt](lr){2-3}  \cmidrule[0.5pt](lr){4}
%                   & EvoDiff        & DPLM                       & DPLM   \\
\multirow{2}{*}{} & \multicolumn{2}{c}{{seq-only}} & \multicolumn{1}{c}{{struct-cond.}} \multicolumn{2}{c}{{ESM3}}  \\ 
\cmidrule[0.5pt](lr){2-3} \cmidrule[0.5pt](lr){4-4} 
                  & EvoDiff        & DPLM &                   \multicolumn{1}{c}{RFDiffusion} &  \\
\midrule
1bcf              & 0.38           & \textbf{1.00}         & \textbf{1.00}       &                              \\
1prw              & 0.36           & \textbf{0.75}        & \textbf{0.81}        &               \\
1qjg              & 0.00              & 0.00                     &0.00           &                           \\
1ycr              & 0.03           & \textbf{0.27}         & \textbf{0.48}       &                \\
2kl8              & 0.00              & \textbf{0.01}        & \textbf{0.01}            &                  \\
3ixt              & 0.09           & \textbf{0.15}                  &  \textbf{0.37}           &           \\
4jhw              & 0.00              & 0.00                    & 0.00                            &          \\
4zyp              & 0.00              & 0.00
&  \textbf{0.01}          &                       \\
5ius              & 0.00              & 0.00
& 0.00                   &     \\
5tpn              & 0.00              & 0.00                    & 0.00                             &      \\
5trv              & 0.00              & 0.00                    & 0.00                            &       \\
5wn9              & 0.00              & 0.00
& 0.00                    &      \\
5yui              & 0.05           & \textbf{0.94}        &  \textbf{0.94}             &             \\
6e6r              & 0.03           & \textbf{0.79}        &  \textbf{0.79}             &          \\
6exz              & 0.00              & \textbf{0.01}        &  \textbf{0.01}             &                   \\
6vw1              & 0.00           & 0.00                    & 0.00                           &        \\
7mrx              & 0.00              & \textbf{0.54}        &  \textbf{0.54}              &         \\ 
\midrule
pass rate         & 6/17           & \textbf{9/27}       &  \textbf{10/17}             &                 \\
avg. success rate & 0.06           & \textbf{0.26}        &  \textbf{0.29}               &                \\ 
\bottomrule
\end{tabular}
}
\vspace{4mm}
\end{table}

==> tables/tokenizer.tex <==
\begin{wrapfigure}[9]{r}{0.45\textwidth}
    \centering
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \begin{table}[H]
           \setlength{\tabcolsep}{2.5pt}
           \small
            \centering
                \resizebox{\textwidth}{!}{
            \begin{tabular}{lrrrrr}
            \toprule
                \multirow{2}{*}{tokenizer} & \multirow{2}{*}{size} & \multicolumn{1}{c}{train}    & \multicolumn{3}{c}{cameo 2022}                                                         \\
                                           &                               & \multicolumn{1}{c}{lddt\_ca} & \multicolumn{1}{c}{lddt\_ca} & \multicolumn{1}{c}{tm-score} & \multicolumn{1}{c}{rmsd} \\
                \midrule
                VQ-VAE-1k                  & 1024                          & 0.76                         & 0.71                         & 0.80                          & 6.14                     \\
                LFQ-1k                     & 1024                          & 0.82                         & 0.77                         & 0.86                         & 4.35                     \\
                LFQ-2k                     & 2048                          & 0.84                         & 0.79                         & 0.88                         & 3.62                     \\
                LFQ-4k                     & 4096                          & 0.86                         & 0.82                         & 0.91                         & 3.31                     \\
                LFQ-8k                     & 8192                          & 0.92                         & 0.86                         & 0.93                         & 2.58                     \\
                LFQ-16k                    & 16384                         & 0.92                         & 0.87                         & 0.94                         & 2.32    \\
                \bottomrule
            \end{tabular}
            }
            % \caption{Sample Table}
        \end{table}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tokenizer-ssp.pdf}
        % \caption{Sample Figure}
    \end{minipage}
\end{wrapfigure}

